Place Deduplication with Embeddings

Thanks to the advancing mobile location services, people nowadays can post about places to share visiting experience on-the-go. A large place graph not only helps users explore interesting destinations, but also provides opportunities for understanding and modeling the real world. To improve coverage and flexibility of the place graph, many platforms import places data from multiple sources, which unfortunately leads to the emergence of numerous duplicated places that severely hinder subsequent location-related services. In this work, we take the anonymous place graph from Facebook as an example to systematically study the problem of place deduplication: We carefully formulate the problem, study its connections to various related tasks that lead to several promising basic models, and arrive at a systematic two-step data-driven pipeline based on place embedding with multiple novel techniques that works significantly better than the state-of-the-art.

==> sec-exp.tex <==
%!TEX root = dedup.tex
\section{Experiments}
\label{sec:exp}
In this section, we take the anonymous real-world place graph from Facebook to comprehensively evaluate our place deduplication pipeline.

\subsection{Experimental Setup}
\subsubsection{Evaluation Metrics}

\subsubsection{Baselines}

\subsection{Experimental Results}
\subsubsection{Feature Analysis}
\subsubsection{Impact of Losses}
\subsubsection{Impact of Hard Sampling}
\subsubsection{Impact of Attentive Training}
\subsubsection{Impact of Label Noise Reduction}

%Motivated by our user type analysis and the correlations between user types and churn, we aim to develop an efficient algorithm for interpretable new user churn prediction. 
%Our analysis of real data shows that new users are most likely to churn in the very beginning of their journey, which urges us to develop an algorithm for fast-response churn prediction. The goal is to accurately predict the likelihood of churn by looking at users' very initial behaviors, while also providing insight into possible reasons behind their churn.
%
%\subsection{Challenges}
%New user churn prediction with high accuracy and limited data is challenging mainly for the following three reasons.
%
%{\flushleft \textbf{Challenge 1: Modeling sequential behavior data.}}
%As we discuss in Section \ref{sec:data}.1, we model each new user by their initial interactions with different functions of the social app as well as their friends, and we collect a 12-dimensional time series $\mathbf{A}_i$ for each new user $u_i \in \mathcal{U}$. However, unlike for user clustering where we leverage the full two-week behavior data of each user, for fast-response churn prediction, we only focus on users' very limited behavior data, \ie, from the initial few days. The data are naturally sequential with temporal dependencies and variable lengths. Moreover, the data are very noisy and bursty. These characteristics pose great challenges to traditional time series models like HMM.
%
%{\flushleft \textbf{Challenge 2: Handling sparse, skewed and correlated activities.}}
%The time series activity data generated by each new user are multi-dimensional. As we show in Section \ref{sec:clustering}, such activity data are very sparse. For example, \textit{Chatters} are usually only active in the first four dimensions as described in Table \ref{tab:act}, while \textit{Sleepers} and \textit{Invitees} are inactive in most dimensions. Even \textit{All-star} users have a lot of 0's in certain dimensions. Besides the many 0's, the distributions of activity counts are highly skewed instead of uniform and many activities are correlated, like we discuss in Section \ref{sec:clustering}.1. 
%%Such properties cannot be well modeled by simple algorithms like logistic regression.
%
%{\flushleft \textbf{Challenge 3: Leveraging underlying user types.}}
%As shown in our new user clustering analysis and highlighted in Figure \ref{fig:type} (b), our clustering of new users is highly indicative of user churn and should be leveraged for better churn prediction. However, as we only get access to initial several days instead of the whole two-week behaviors, user types are also unknown and should be jointly inferred with user churn. Therefore, how to design the proper model that can simultaneously learn the patterns for predicting user types and user churn poses a unique technical challenge that cannot be solved by existing approaches.
%
%\subsection{Methods and Results}
%We propose a series of solutions to treat the challenges listed above. Together they form our efficient churn prediction framework.
%We also present comprehensive experimental evaluations for each proposed model component. Our experiments are done on an anonymous internal dataset of Snapchat, which includes 37M users and 697M bi-directional links.
%The metrics we compute include accuracy, precision, and recall, which are commonly used for churn prediction and multi-class classification \cite{tsoumakas2006multi}.
%The baselines we compare with are logistic regression and random forest, which are the standard and most widely practiced models for churn prediction and classification. %We also compare with HMM, which is the standard model for learning with time series data.
%We randomly split the new user data into training and testing sets with the ratio 8:2 for 10 times, and run all compared algorithms on the same splits to take the average performance for evaluation.
%All experiments are run on a single machine with a 12-core 2.2GHz CPU and no GPU, although the runtimes of our neural network models can be largely improved on GPUs.
%
%{\flushleft \textbf{Solution 1: Sequence-to-sequence learning with LSTM.}}
%The intrinsic problem of user behavior understanding is sequence modeling. The goal is to convert sequences of arbitrary lengths with temporal dependences into a fixed-length vector for further usage. To this end, we propose to leverage the state-of-the-art sequence-to-sequence model, that is, LSTM  (Long-Short Term Memory) from the family of RNN (Recurrent Neural Networks) \cite{hochreiter1997long, mikolov2010recurrent}. Specifically, we apply a standard multi-layer LSTM to the multi-dimensional input $\mathbf{A}$. Each layer of the LSTM computes the following functions
%\begin{align}
%i_t&=\sigma(W_i\cdot[h_{t-1}, x_t]+b_i) \\\nonumber
%f_t&=\sigma(W_f\cdot[h_{t-1}, x_t]+b_f) \\\nonumber
%c_t&=f_t*c_{t-1}+i_t*\text{tanh}(W_c\cdot[h_{t-1}, x_t]+b_c) \\\nonumber
%o_t&=\sigma(W_o\cdot[h_{t-1}, x_t]+b_o) \\\nonumber
%h_t&=o_t*\text{tanh}(c_t)
%\end{align}
%where $t$ is the time step in terms of days, $h_t$ is the hidden state at time $t$, $c_t$ is the cell state at time $t$, $x_t$ is the hidden state of the previous layer at time $t$, with $x_t=a_{\cdot t}$ for the first layer, and $i_t$, $f_t$, $o_t$ are the input, forget and out gates, respectively. $\sigma$ is the sigmoid function $\sigma(x)=1/(1+e^{-x})$. Dropout is also applied to avoid overfitting. We use $\Theta_l$ to denote the set of parameters in all LSTM layers.
%
%A linear projection with a sigmoid function is connected to the output of the last LSTM layer to produce user churn prediction as
%\begin{align}
%\hat{y} = \sigma(\mathbf{W}_c o_T+\mathbf{b}_c).
%\label{eq:linear}
%\end{align}
%We use $\Theta_c$ to denote the parameters in this layer, \ie, $\mathbf{W}_c$ and $\mathbf{b}_c$.
%
%Unlike standard methods for churn prediction such as logistic regression or random forest, LSTM is able to model user behavior data as time series and capture the evolvement of user activities through recognizing the intrinsic temporal dependencies. Furthermore, compared with standard time series models like HMM, LSTM is good at capturing both long term and short term dependences within sequences of variable lengths. When the lengths are short, LSTM acts similarly as basic RNN  \cite{mikolov2010recurrent}, but when more user behaviors become available, LSTM is expected to excel. 
%
%Figure \ref{fig:exp} (a) shows the performances of compared models. 
%The length of the output sequence of LSTM is empirically set to 64. 
%In the experiments, we vary the amounts of user behavior data the models get access to and find that more days of behavior data generally lead to better prediction accuracy. We can also see that new users' initial activities in the first few days are more significant in improving the overall accuracy. A simple LSTM model can outperform all compared baselines with a substantial margin. The runtime of LSTM on CPU is within ten times of the runtimes of other baselines, and it can be significantly improved on GPUs.
%
%\begin{figure*}[h!]
%\centering
%\vspace{-20pt}
%\subfigure[Single LSTM]{
%\includegraphics[width=0.235\textwidth]{figures/fig_exp1.png}}
%\subfigure[Activity embedding]{
%\includegraphics[width=0.235\textwidth]{figures/fig_exp2.png}}
%\subfigure[Parallel LSTMs]{
%\includegraphics[width=0.235\textwidth]{figures/fig_exp3.png}}
%\subfigure[User type prediction]{
%\includegraphics[width=0.26\textwidth]{figures/fig_exp4.pdf}}
%\caption{\textbf{Comprehensive experimental results on our churn prediction framework compared with various baseline methods.}}
%\label{fig:exp}
%\end{figure*}
%
%{\flushleft \textbf{Solution 2: LSTM with activity embedding.}}
%To deal with sparse, skewed and correlated activity data, we propose to add an activity embedding layer in front of the standard LSTM layer. Specifically, we connect a fully connected feedforward neural network to the original daily activity vectors, which converts users' sparse activity features of each day into distributional activity embeddings, while deeply exploring the skewness and correlations of multiple features through the linear combinations and non-linear transformations. 
%Specifically, we have
%\begin{align}
%e_{\cdot t} = \psi^H(\ldots\psi^2(\psi^1(a_{\cdot t}))\ldots),
%\end{align}
%where
%\begin{align}
%\psi^h(e) = \text{ReLU}(W_e^h \text{Dropout}(e)+b^h_e).
%\end{align}
%$H$ is the number of hidden layers in the activity embedding network. $\Theta_e$ is the set of parameters in these $H$ layers.
%With the activity embedding layers, we simply replace $\mathbf{A}$ by $\mathbf{E}$ for the input of the first LSTM layer, with the rest of the architectures unchanged.
%
%Figure \ref{fig:exp} (b) shows the performances of LSTM with activity embedding of varying number of embedding layers and embedding sizes. 
%The length of the output sequence of LSTM is kept as 64.
%The overall performances are significantly improved with one single layer of fully connected non-linear embedding (\textit{LSTM+1}), while more layers (\eg, \textit{LSTM+2}) and larger embedding sizes tend to yield similar performances. The results are intuitive because a single embedding layer is usually sufficient to deal with the sparsity, skewness, and correlations of daily activity data. We do not observe significant model overfitting due to the dropout technique and the large size of our data compared with the number of model parameters.
%
%{\flushleft \textbf{Solution 3: Parallel LSTMs with joint training.}}
%To further improve our churn prediction, we pay attention to the underlying new user types. The idea is that, for users in the training set, we get their two-week behavior data, so besides computing their churn labels $y$ based on their second-week activities, we can also compute their user types $\mathbf{t}$ with our clustering framework. For users in the testing set, we can then compare the initial behaviors with those in the training set to guess their user types, and leverage the correlation between user types and churn for better churn prediction.
%
%To implement this idea, we propose parallel LSTMs with joint training. Specifically, we assume there are $K$ user types. $K$ can be either chosen automatically by our clustering framework or set to specific values. Then we jointly train $K$ sub-LSTMs on the training set. Each sub-LSTM is good at modeling one type of users. We parallelize the $K$ sub-LSTMs and merge them through attention \cite{denil2012learning} to jointly infer hidden user types and user churn.
%
%\begin{figure}[h!]
%    \includegraphics[width=1\linewidth]{figures/fig_plstm.pdf}
%    \caption{\small Parallel LSTMs with user type attention.}
%    \label{fig:plstm}
%\end{figure}
%
%As shown in Figure \ref{fig:plstm}, for each user, the input of a sequence of activity embedding vectors $\mathbf{E}$ is put into $K$ sub-LSTMs in parallel to generate $K$ \textit{typed sequences}:
%\begin{align}
%\mathbf{s}_k = \text{LSTM}_k(\mathbf{E}).
%\end{align}
%
%To differentiate hidden user types and leverage this knowledge to improve churn prediction, we introduce an attention mechanism to generate user behavior embeddings by focusing on their latent types. A positive attention weight $w_k$ is placed on each user type to indicate the probability of the user to be of a particular type. We compute $w_k$ as a similarity of the corresponding typed sequence $\mathbf{s}_k$ and a global unique \textit{typing vector} $\mathbf{v}_t$, which is jointly learned during the training process. 
%\begin{align}
%w_k=\text{softmax}(\mathbf{v}_t^T \mathbf{s}_k).
%\end{align}
%Here \textsf{softmax} is taken to normalize the weights and is defined as $\text{softmax}(x_i)=\frac{\text{exp}(x_i)}{\sum_j \text{exp}(x_j)}$.
%The user behavior embedding $\mathbf{u}$ is then computed as a sum of the typed sequences weighted by their importance weights:
%\begin{align}
%\mathbf{u}=\sum_{k=1}^K w_k \mathbf{s}_k.
%\end{align}
%The same linear projection with sigmoid function as in Eq.~\ref{eq:linear} is connected to $\mathbf{u}$ to predict user churn as binary classification.
%\begin{align}
%\hat{y} = \sigma(\mathbf{W}_c \mathbf{u}+\mathbf{b}_c).
%\end{align}
%
%To leverage user types for churn prediction, we jointly train a typing loss $l_t$ and a churn loss $l_c$.
%For $l_t$, we firstly compute users' soft clustering labels $\mathbf{Q}$ as
%\begin{align}
%q_{ik} = \frac{(1+||\mathbf{f}_i-\mathbf{c}_k||^2)^{-1}}{\sum_j(1+||\mathbf{f}_i-\mathbf{c}_j||^2)^{-1}}.
%\end{align}
%$q_{ik}$ is a kernel function that measures the similarity between the feature $\mathbf{f}_i$ of user $u_i$ and the cluster center $\mathbf{c}_k$. It is computed as the probability of assigning $u_i$ to the $k$th type, under the assumption of Student's $t$-distribution with degree of freedom set to 1 \cite{maaten2008visualizing}.
%
%We use $w_{ik}$ to denote the attention weight for user $u_i$ on type $t_k$. Thus, for each user $u_i$, we compute her typing loss as the cross entropy on $q_{i\cdot}$ and $w_{i\cdot}$. So we have
%\begin{align}
%l_t=-\sum_i \sum_k q_{ik}\log(w_{ik}).
%\end{align}
%For $l_c$, we simply compute the log loss for binary predictions as
%\begin{align}
%l_c=\sum -y_i \log\hat{y}_i - (1-y_i)\log(1-\hat{y}_i),
%\end{align}
%where $y_i$ is the binary ground-truth churn label and $\hat{y}_i$ is the predicted churn label for user $u_i$, respectively.
%
%Subsequently, the overall objective function of our parallel LSTM with joint training is 
%\begin{align}
%l=l_c+\lambda l_t,
%\end{align}
%where $\lambda$ is a hyper-parameter controlling the trade-off between churn prediction and type prediction. We empirically set it to a small value like 0.1 in our experiments.
%
%Figure \ref{fig:exp} (c) shows the performances of parallel LSTMs with and without joint training (\textit{PLSTM}+ vs.~\textit{PLSTM}). The only difference between the two frameworks is that \textit{PLSTM} is not trained with the correct user types produced by our clustering framework. In the experiments, we vary the number of clusters and sub-LSTMs and find that joint training is always significantly helpful. The performance of parallel LSTMs with joint training peaks with 3 or 6 sub-LSTMs. While the number 3 may accidentally align with some trivial clusters, the number 6 actually aligns with the six interpretable cohorts automatically chosen by our clustering framework, which illustrates the coherence of our two frameworks and further supports the sanity of splitting the new users into six types.
%
%Besides churn prediction, Figure \ref{fig:exp} (d) shows that we can also predict what type a new user is by looking at her initial behaviors rather than two-week data, with different precisions and recalls. Our algorithm is good at capturing \textit{All-star}, \textit{Sleeper} and \textit{Invitee}, due to their distinct behavior patterns. \textit{Swiper} and \textit{Bumper} are harder to predict because their activity patterns are less regular. Nonetheless, such fast-response churn predictions with insights into user types can directly enable many actionable production decisions such as fast retention and targeted promotion. 


==> sec-pipeline.tex <==
%!TEX root = dedup.tex
\section{Our Pipeline}
\label{sec:pipeline}
%Motivated by recent success in embedding and representation learning, in this work, we aim to learn high-quality place embeddings for efficient place deduplication. The data we can leverage mainly includes two parts: 1) ad-hoc place attributes and 2) noisy labeled place pairs. Driven by the particular problem and data at hand, we propose a systematic two-step embedding pipeline consisting of large-scale unsupervised feature generation and efficient supervised metric learning. 


